Towards Optimal Off-Policy Evaluation for Reinforcement Learning with Marginalized Importance Sampling

Motivated by the many real-world applications of reinforcement learning (RL) that require safe-policy iterations, we consider the problem of off-policy evaluation (OPE) -- the problem of evaluating a new policy using the historical data obtained by different behavior policies -- under the model of nonstationary episodic Markov Decision Processes (MDP) with a long horizon and a large action space. Existing importance sampling (IS) methods often suffer from large variance that depends exponentially on the RL horizon $H$. To solve this problem, we consider a marginalized importance sampling (MIS) estimator that recursively estimates the state marginal distribution for the target policy at every step. MIS achieves a mean-squared error of $$ \frac{1}{n} \sum\nolimits_{t=1}^H\mathbb{E}_{\mu}\left[\frac{d_t^\pi(s_t)^2}{d_t^\mu(s_t)^2} \mathrm{Var}_{\mu}\left[\frac{\pi_t(a_t|s_t)}{\mu_t(a_t|s_t)}\big( V_{t+1}^\pi(s_{t+1}) + r_t\big) \middle| s_t\right]\right] + \tilde{O}(n^{-1.5}) $$ where $\mu$ and $\pi$ are the logging and target policies, $d_t^{\mu}(s_t)$ and $d_t^{\pi}(s_t)$ are the marginal distribution of the state at $t$th step, $H$ is the horizon, $n$ is the sample size and $V_{t+1}^\pi$ is the value function of the MDP under $\pi$. The result matches the Cramer-Rao lower bound in \citet{jiang2016doubly} up to a multiplicative factor of $H$. To the best of our knowledge, this is the first OPE estimation error bound with a polynomial dependence on $H$. Besides theory, we show empirical superiority of our method in time-varying, partially observable, and long-horizon RL environments.

==> sections/app_proof_2.tex <==
% !TEX root = ../paper.tex

\section{Proof Details of Section~\ref{sec:estratio}}
\label{app:proof_sec4}

% For the moment, assume $\mu(s_t)$ is known.

% Let 
% \begin{align}
% \widetilde \pi(s_t) = & \pi(s_t) + \varepsilon(s_t) \\
% \widehat \pi(s_t) = & \frac{\pi(s_t) + \varepsilon(s_t)}{1 + \sum \varepsilon(s_t)},
% \end{align}
% where $\varepsilon(s_t)$ satisfies $\varepsilon(s_t) \geq -\pi(s_t)$ and $\sum \varepsilon(s_t) \geq -1$. Then,
% \begin{align}
% \widetilde \pi(s_{t+1}) = & \frac{1}{n} \sum_{i = 1}^{n}\frac{\widehat \pi(s_t^i)}{\mu(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s_{t+1}) \\
% = & \frac{1}{1 + \sum \varepsilon(s_t)} \left[ \frac{1}{n}\sum_{i = 1}^{n} \frac{\pi(s_t^i)}{\mu(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s_{t+1}) + \frac{1}{n}\sum_{i = 1}^{n} \frac{\varepsilon(s_t^i)}{\mu(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s_{t+1}) \right] \\
% = & \frac{1}{1 + \sum \varepsilon(s_t)} \Bigg[ \pi(s_{t+1}) + O\left( \frac{\sqrt{\mathbb E_{\mu} (\rho_t^2)}}{\sqrt{n}} \right) + \sum_{s_t} \underbrace{\frac{1}{n} \sum_{i = 1}^{n} \frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)} \mathbf 1(s_{t + 1}^i = s_{t + 1}, s_{t}^i = s_t)}_{= \mathbb P_{\pi}(s_{t+1}|s_t)\mu_{s_t} + O\left( \frac{\sqrt{\mathbb E_{\mu} [\rho_{t,a}^2]}}{\sqrt{n}} \right)} \frac{\varepsilon(s_t)}{\mu(s_t)} \Bigg] \\
% = & \frac{1}{1 + \sum \varepsilon(s_t)} \left[ \pi(s_{t+1}) + \sum_{s_t} \mathbb P_{\pi}(s_{t+1}|s_t) \varepsilon(s_t) + O\left( \frac{\sqrt{\mathbb E_{\mu} [\rho_{t}^2]}}{\sqrt{n}} + \frac{\sqrt{\max_{s_t} \mathbb E_{\mu} [\rho_{t,a}^2]} }{\sqrt{n}} \varepsilon(s_t) \right)\right].
% \end{align}
% Note that, the difference between normalized and unnormalized version is whether there is a $\frac{1}{1 + \sum \varepsilon(s_t)}$ term.

% We now discuss the $\varepsilon(s_t)$ term for the unnormalized case.
% \begin{align}
% \varepsilon(s_{t+1}) = & \sum_{s_t} \mathbb P_{\pi}(s_{t+1}|s_t)\varepsilon(s_t) + O\left( \frac{\sqrt{\mathbb E_{\mu} [\rho_{t}^2]}}{\sqrt{n}} + \frac{\sqrt{\max_{s_t} \mathbb E_{\mu} [\rho_{t,a}^2 | s_t]} }{\sqrt{n}} \sum_{s_t} \varepsilon(s_t) \right) \\
% |\varepsilon(s_{t+1})| \leq & \sum_{s_t} \mathbb P_{\pi}(s_{t+1}|s_t) |\varepsilon(s_t)| + O\left( \frac{\sqrt{\mathbb E_{\mu} [\rho_{t}^2]}}{\sqrt{n}} + \frac{\sqrt{\max_{s_t} \mathbb E_{\mu} [\rho_{t,a}^2 | s_t]} }{\sqrt{n}} \sum_{s_t} |\varepsilon(s_t)| \right).
% \end{align}
% Take summation over $s_{t+1}$ on both sides, we have the following results for the unnormalized version,
% \begin{align}
% \sum_{s_{t+1}}|\varepsilon(s_{t+1})| \leq & \sum_{s_{t}} |\varepsilon(s_{t})| + O\left( \frac{|\mathcal S|\sqrt{\mathbb E_{\mu} [\rho_{t}^2]}}{\sqrt{n}} + \frac{|\mathcal S|\sqrt{\max_{s_t} \mathbb E_{\mu} [\rho_{t,a}^2 | s_t]} }{\sqrt{n}} \sum_{s_t} |\varepsilon(s_{t})| \right) \\
% \Rightarrow \sum_{s_{t+1}}|\varepsilon(s_{t+1})| \leq & \left( 1 + O\left(\frac{|\mathcal S|\sqrt{\max_{s_t} \mathbb E_{\mu} [\rho_{t,a}^2 | s_t]} }{\sqrt{n}} \right) \right)\sum_{s_{t}}|\varepsilon(s_{t})| + \frac{\sqrt{\mathbb E_{\mu} [\rho_{t}^2]}}{\sqrt{n}}.
% \end{align}
% %
% %\note[tx]{I modified a little for the (in)equation above}
% %
% Thus, if $\sum_{s_{t}} |\varepsilon(s_{t})| \leq 1$, the error grows linearly; and if $\sum_{s_{t}}|\varepsilon(s_{t})| > 1$, the error grows exponentially but with a small factor. Since that, we can handle horizon up to $H = {\sqrt{n}}/{\sqrt{\mathbb{E} [\rho_t^2]}}$.

% For the case with normalization, $\varepsilon(s_{t+1})$ becomes different
% \begin{align}
% \varepsilon(s_{t+1}) = & -\pi(s_{t+1}) + \frac{1}{n} \sum_{i = 1}^{n}\frac{\widehat \pi(s_t^i)}{\mu(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s_{t+1}) \\
% = & -\pi(s_{t+1}) + \frac{1}{1 + \sum \varepsilon (s_t)} \left( \pi(s_{t+1}) + O\left( \frac{\sqrt{\mathbb E [\rho_t^2]}}{\sqrt{n}} \right) \right) \\
% & + \frac{1}{1 + \sum \varepsilon (s_t)} \left( \sum_{s_t} \mathbb P_{\pi}(s_{t+1}|s_t)\varepsilon(s_t) + O\left( \frac{\sqrt{\mathbb E_{\mu}[\rho_{t,a}^2]}}{\sqrt{n}} |\varepsilon (s_t)| \right) \right) \\
% = & \left(-1 + \frac{1}{1 + \sum \varepsilon (s_t)}\right) \pi(s_{t+1}) + \frac{\sum_{s_t}P_{\pi}(s_{t+1}|s_t)\varepsilon(s_t)}{1 + \sum \varepsilon (s_t)} \\
% & + \frac{1}{1 + \sum \varepsilon (s_t)} O\left( \frac{\sqrt{\mathbb E_{\mu}[\rho_{t}^2]}}{\sqrt{n}} + \frac{\sqrt{\mathbb E_{\mu}[\rho_{t,a}^2]}}{\sqrt{n}} |\varepsilon (s_t)|\right).
% \end{align}
% Let's first calculate $\sum_{s_{t+1}} \varepsilon (s_{t+1})$
% \begin{align}
% \sum_{s_{t+1}} \varepsilon (s_{t+1}) = -\frac{\sum \varepsilon(s_t)}{1 + \sum \varepsilon(s_t)} + \frac{\sum \varepsilon(s_t)}{1 + \sum \varepsilon(s_t)} + O\left( \frac{|\mathcal S_{t+1}| \left(\sqrt{\mathbb E_{\mu}[\rho_{t}^2]} + \sqrt{\mathbb E_{\mu}[\rho_{t,a}^2]} |\varepsilon (s_t)| \right)}{\sqrt{n} (1 + \sum \varepsilon (s_t))}  \right).
% \end{align}
% Thus, when $|\varepsilon(s_t)| \leq 1$, it takes 
% \begin{align}
% H \asymp \frac{\sqrt{n}}{|\mathcal S| \left(\sqrt{\mathbb E_{\mu}[\rho_{t}^2]} + \sqrt{\mathbb E_{\mu}[\rho_{t,a}^2]} |\varepsilon (s_t)| \right)}
% \end{align}
% before $\sum_{s_{t+1}}\varepsilon(s_{t+1})$ could reach $-0.5$.

% Now
% \begin{align}
% \|\varepsilon(s_{t+1})\|_1 \leq \frac{\|\varepsilon(s_t)\|_1}{1 + \sum \varepsilon(s_t)} + \frac{|\mathcal S_{t+1}||\sum_{s_t}\varepsilon(s_t)|}{1 + \sum \varepsilon(s_t)} + O \left( \frac{ |\mathcal S_{t+1}| \left(\sqrt{\mathbb E_{\mu}[\rho_{t}^2]} + \sqrt{\mathbb E_{\mu}[\rho_{t,a}^2]} |\varepsilon (s_t)| \right)}{\sqrt{n} (1 + \sum \varepsilon (s_t))} \right).
% \end{align}

% Collecting the bounds we get:
% \begin{align}
% |\varepsilon(s_{t+1})| \leq & \left( \frac{1 + \frac{|\mathcal S_{t+1}|\sqrt{ \mathbb E_{\mu}[\rho_{t,a}^2]}}{\sqrt{n}}}{1 + \sum \varepsilon (s_t)} \right) |\varepsilon(s_{t})| + \frac{|\mathcal S_{t+1}|^2 \sqrt{\mathbb E_{\mu}[\rho_{t}^2]}}{\sqrt{n} (1 + \sum \varepsilon (s_t))^2} \\
% & +  \frac{|\mathcal S_{t+1}|^2 \sqrt{\mathbb E_{\mu}[\rho_{t,a}^2]}}{\sqrt{n} (1 + \sum \varepsilon (s_t)))^2} |\varepsilon(s_t)| + \frac{|\mathcal S_{t+1}| \sqrt{\mathbb E_{\mu}[\rho_{t}^2]}}{\sqrt{n} (1 + \sum \varepsilon (s_t))}
% \end{align}

% This is quantitatively the same as the version without normalization. But it strictly reduces the error if $(1 + \sum \varepsilon (s_t)) > 1$.

% Thus our \textit{idea} is: choose unnormalized version if $(1 + \sum \varepsilon (s_t)) < 1$, otherwise choose the normalized version. Note that $(1 + \sum \varepsilon (s_t)) < 1 \iff \sum \tilde \pi (s_t) < 1$.


% \subsection{Full version}

In this section, we provide the details proof in the part of marginalized density ratio estimation. 

Before we start our proof, we review the assumptions we made about $\pi, \mu, d_t^{\mu}, d_t^{\pi}$. Assume there exists $\eta > 0$, such that $\pi(a|s) / \mu(a|s) \leq 1 / \eta$ for any $(s,a)$. We also assume there exists $\{\eta_t > 0\}_{t = 0}^{H - 1}$, such that $d_t^{\mu}(s) \geq \eta_t$ for all $s$ and $t$. we first prove  Theorem \ref{thm:err_prop_1}.

\begin{proof}[Proof of Theorem \ref{thm:err_prop_1}]

% \paragraph{Non-normalized case:}

Given the definition of the non-normalized estimation $\widehat d_{t}^{\pi}(s_t^i)$ in \eqref{eq:dpirecest1}, we have
\begin{align}
& \widehat d_{t + 1}^{\pi}(s) \\
= & \frac{1}{n} \sum_{i = 1}^{n}\frac{\widehat d_{t}^{\pi}(s_t^i)}{\widehat d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \\
= & \frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i) + \varepsilon_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i) + \varepsilon_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \\
= & \frac{1}{n} \sum_{i = 1}^{n} \left(\frac{(d_{t}^{\pi}(s_t^i) + \varepsilon_{t}^{\pi}(s_t^i)) (d_{t}^{\mu}(s_t^i) - \varepsilon_{t}^{\mu}(s_t^i))}{(d_{t}^{\mu}(s_t^i))^2 - (\varepsilon_{t}^{\mu}(s_t^i))^2} \right) \frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \\
= & \frac{1}{n} \sum_{i = 1}^{n} \left(\frac{(d_{t}^{\pi}(s_t^i) + \varepsilon_{t}^{\pi}(s_t^i)) (d_{t}^{\mu}(s_t^i) - \varepsilon_{t}^{\mu}(s_t^i))}{(d_{t}^{\mu}(s_t^i))^2} + \frac{d_{t}^{\pi}(s_t^i)}{(d_{t}^{\mu}(s_t^i))^3} \widetilde{\mathcal O}\left( \frac{1}{n} \right) \right) \frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \\
%
%
%
= & \underbrace{\frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \left(1 + \widetilde{\mathcal O}\left( \frac{1}{n}\right)\right)}_{\text{(a)}} + \underbrace{\frac{1}{n} \sum_{i = 1}^{n}\frac{\varepsilon_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s)}_{\text{(b)}} \\
& + \underbrace{\frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i) \varepsilon_{t}^{\mu}(s_t^i)}{(d_{t}^{\mu}(s_t^i))^2}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s)}_{\text{(c)}} + \underbrace{\frac{1}{n} \sum_{i = 1}^{n}\frac{\varepsilon_{t}^{\pi}(s_t^i) \varepsilon_{t}^{\mu}(s_t^i)}{(d_{t}^{\mu}(s_t^i))^2}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s)}_{\text{(d)}},
\end{align}
where the all inequalities above are calculated by the direct simplification.

We now analyze these four terms above separately. For the term (a):
\begin{align}
& \frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \left(1 + \widetilde{\mathcal O}\left( \frac{1}{n}\right)\right) \\
= & \left( d_{t + 1}^{\pi}(s) + \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \right) \right)  \left(1 + \widetilde{\mathcal O}\left( \frac{1}{n}\right)\right) \\
= & d_{t + 1}^{\pi}(s) + \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \right),
\label{eq:terma}
\end{align}
where $w_t(s) = d_t^{\pi}(s) / d_t^{\mu}(s)$.


In the above derivation, we applied Hoeffding's inequality on
$$
\frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) - \E \left[\frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s)\right].
$$

We first calculate the expectation, where $a_t^i, s_{t}^i,s_{t+1}^i$ are sampled by behavior policy $\mu$.
\begin{align}
\E_{\mu} \left[\frac{d_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s)\right] = & \int  p_{\mu}(s_t^i, s_{t+1}^i, a_t^i) \frac{d_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s)  d(s_t^i, s_{t+1}^i, a_t^i)\\
=&\int p(s_{t+1}^i | s_t^i, a_t^i) p_{\mu}(s_t^i) \mu(a_t^i|s_t^i)  \frac{d_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) d(s_t^i, s_{t+1}^i, a_t^i) \\
=&\int p(s_{t+1}^i | s_t^i, a_t^i)  d_{t}^{\pi}(s_t^i) \pi(a_t^i|s_t^i) \mathbf 1(s_{t+1}^i = s) d(s_t^i, s_{t+1}^i, a_t^i) \\
=& \mathbb E_{\pi} [\mathbf 1(s_{t+1}^i = s)]\\
=& d_{t + 1}^{\pi}(s)
\end{align}

Then, by Hoeffding's inequality we have that with probability $1-\delta$
\begin{align}
&\left| \frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) - \E \left[\frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s)\right]\right|
%= & O\left( \left(\sqrt{\frac{\E_\mu\left[(\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)})^2\middle| s_{t}^i = s_t, s_{t+1}^i = s\right] p_\mu\left[s_t\right]p_\mu\left[s|s_t\right] }{n}  }  +  \frac{1}{\eta n} \right)\log(1/\delta)  \right)\\
\leq O\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \log(1/\delta)\right)
\end{align}

For the term (b):
\begin{align}
& \frac{1}{n} \sum_{i = 1}^{n}\frac{\varepsilon_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \\
= & \sum_{s_t}\frac{1}{n} \sum_{i = 1}^{n}\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)}\mathbf 1(s_{t}^i = s_t, s_{t+1}^i = s) \frac{\varepsilon_{t}^{\pi}(s_t)}{d_{t}^{\mu}(s_t)} \\
= & \sum_{s_t} d_{t}^{\mu}(s_t) \left[ \mathbb P_{\pi}(s|s_t) + \widetilde{\mathcal O}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right)\right] \frac{\varepsilon_{t}^{\pi}(s_t)}{d_{t}^{\mu}(s_t)}
% = & \sum_{s_t} \left[ \mathbb P_{\pi}(s|s_t) + \widetilde{\mathcal O}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \right] \varepsilon_{t}^{\pi}(s_t)
\label{eq:termb}
\end{align}
% \note[tx]{Not sure if the Big-O term above also need a $1 / d_t^{\mu}$}

% \note[yw]{ At the moment, yes,  but it's fine.  I have an argument to make it cleaner. But I'll have to go pick up my son.}

In the above derivation, we applied Bernstein's inequality on
$$
\frac{1}{n} \sum_{i = 1}^{n}\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)}\mathbf 1(s_{t}^i = s_t, s_{t+1}^i = s) - \E \left[\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)}\mathbf 1(s_{t}^i = s_t, s_{t+1}^i = s)\right].
$$
Let's first calculate the expectation (noted that $a_t^i, s_{t}^i,s_{t+1}^i$ are drawn under policy $\mu$).

\begin{align*}
\E_\mu \left[\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)}\mathbf 1(s_{t}^i = s_t, s_{t+1}^i = s)\right] =& 
\int  p_{\mu}(s_t^i, s_{t+1}^i, a_t^i) \frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)}\mathbf 1(s_{t}^i = s_t, s_{t+1}^i = s)  d(s_t^i, s_{t+1}^i, a_t^i)\\
=&\int p(s_{t+1}^i | s_t^i, a_t^i) p_{\mu}(s_t^i) \mu(a_t^i|s_t^i)  \frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)}  1(s_{t}^i = s_t, s_{t+1}^i = s)  d(s_t^i, s_{t+1}^i, a_t^i) \\
=& \int [\sum_{a_t^i}p(s_{t+1}^i | s_t^i, a_t^i) \pi(a_t^i|s_t) ]  p_{\mu}(s_t^i) \mathbf 1(s_{t}^i = s_t, s_{t+1}^i = s)  d(s_t^i, s_{t+1}^i)\\
=&\sum_{a_t^i}p(s_{t+1}^i=s | s_t, a_t^i) \pi(a_t^i|s_t) ] p_{\mu}(s_t)\\
=&  p_{\pi}(s | s_t)  p_{\mu}(s_t).
\end{align*}
Let's now bound the variance of this random variable.
\begin{align*}
\Var_\mu\left[\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)}\mathbf 1(s_{t}^i = s_t, s_{t+1}^i = s)\right] &\leq \E_\mu\left[(\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)})^2\mathbf 1(s_{t}^i = s_t, s_{t+1}^i = s)\right]\\
&= \E_\mu\left[(\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)})^2\middle| s_{t}^i = s_t, s_{t+1}^i = s\right] p_\mu\left[s_t\right]p_\mu\left[s|s_t\right]\\
&\leq \E_\mu\left[(\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)})^2\mathbf 1(s_{t}^i = s_t)\right]\leq  \E\left[(\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)})^2 \middle| s_t\right]p_{\mu}(s_t).
\end{align*}
% \begin{align*}
%     \Var[\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)}\mathbf 1(s_{t}^i = s_t, s_{t+1}^i = s)]  =&  \E[\Var[\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)}\mathbf 1(s_{t}^i = s_t, s_{t+1}^i = s) | s_{t}^i=s_t,s_{t+1}^i = s]]   + \Var[ \E[\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)}\mathbf 1(s_{t}^i = s_t, s_{t+1}^i = s) | s_{t}^i=s_t,s_{t+1}^i = s]]\\
%     =& d_t^{\mu}(s_{t}^i=s_t,s_{t+1}^i = s) \Var[\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)}] + 
% \end{align*}

By Bernstein's inequality we have that with probability $1-\delta$
\begin{align*}
&\left| \frac{1}{n} \sum_{i = 1}^{n}\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)}\mathbf 1(s_{t}^i = s_t, s_{t+1}^i = s) -  p_{\pi}(s | s_t)  p_{\mu}(s_t)\right| \\
%= & O\left( \left(\sqrt{\frac{\E_\mu\left[(\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)})^2\middle| s_{t}^i = s_t, s_{t+1}^i = s\right] p_\mu\left[s_t\right]p_\mu\left[s|s_t\right] }{n}  }  +  \frac{1}{\eta n} \right)\log(1/\delta)  \right)\\
\leq& O\left(  \left(\sqrt{\frac{\E\left[\rho_t^2 \middle| s_t\right] \P_{\mu}(s_t)}{n}} + \frac{1}{\eta n}  \right) \log(1/\delta)\right)
\end{align*}

% \begin{lemma}
% The function $f(x,y)  =  \sqrt{x}/y$ is jointly concave in $(x,y)\in \R_+^2$.
% \end{lemma}
% \begin{proof}
% The hessian of this function is
% $$
% \begin{bmatrix} 
%  -\frac{x^{-3/2}}{4y}& -\frac{x^{-1/2}}{y^2} \\
%  -\frac{x^{-1/2}}{y^2} & \frac{2 x^{1/2}}{y^3}
% \end{bmatrix} 
% $$
% Find eigenvalue?...  
% \end{proof}



For the term (c):
\begin{align}
& \frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i) \varepsilon_{t}^{\mu}(s_t^i)}{(d_{t}^{\mu}(s_t^i))^2}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \\
= & \frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \frac{\varepsilon_{t}^{\mu}(s_t^i)}{d_{t}^{\mu}(s_t^i)} \\
= & \left( d_{t + 1}^{\pi}(s) + \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \right) \right) \frac{\widetilde{\mathcal O}\left( \frac{1}{\sqrt{n}} \right)}{d_{t}^{\mu}(s_t^i)},
\label{eq:termc}
\end{align}
where the last equality follow from \eqref{eq:terma} and Fact \ref{fct:fct1}.

For the term (d):
\begin{align}
& \frac{1}{n} \sum_{i = 1}^{n}\frac{\varepsilon_{t}^{\pi}(s_t^i) \varepsilon_{t}^{\mu}(s_t^i)}{(d_{t}^{\mu}(s_t^i))^2}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \\
= & \frac{1}{n} \sum_{i = 1}^{n}\frac{\varepsilon_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \frac{\varepsilon_{t}^{\mu}(s_t^i)}{d_{t}^{\mu}(s_t^i)} \\
= & \sum_{s_t} \left[ \mathbb P_{\pi}(s|s_t) + \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \right)\right] \frac{\varepsilon_{t}^{\pi}(s_t) \widetilde{\mathcal O}\left( \frac{1}{\sqrt{n}} \right)}{d_{t}^{\mu}(s_t^i)}
\label{eq:termd}
\end{align}
where the last equality follow from \eqref{eq:termb} and Fact \ref{fct:fct1}.

Combining \eqref{eq:terma}, \eqref{eq:termb}, \eqref{eq:termc} and \eqref{eq:termd}, we obtain
\begin{align}
\widehat d_{t + 1}^{\pi}(s) = & d_{t + 1}^{\pi}(s) + \sum_{s_t} \mathbb P_{\pi}(s|s_t) \varepsilon_{t}^{\pi}(s_t) + \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \right) + \sum_{s_t} \widetilde{\mathcal O}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \varepsilon_{t}^{\pi}(s_t) \\
\label{eq:dhatnonnorm}
\end{align}

According the definition of $\varepsilon_{t + 1}^{\pi}(\cdot)$, we have
\begin{align}
\varepsilon_{t + 1}^{\pi}(s) =  & \sum_{s_t} \mathbb P_{\pi}(s|s_t) \varepsilon_{t}^{\pi}(s_t) + \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + \sum_{s_t}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \varepsilon_{t}^{\pi}(s_t)\right)\\
|\varepsilon_{t + 1}^{\pi}(s)| \leq  & \sum_{s_t} \mathbb P_{\pi}(s|s_t) |\varepsilon_{t}^{\pi}(s_t)| + \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + \sum_{s_t}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) |\varepsilon_{t}^{\pi}(s_t)|\right).
\label{eq:bdsnonnorm}
\end{align}

Taking summation over $s$ on each side of \eqref{eq:bdsnonnorm}, we obtain
% \begin{align}
% \sum_{s} \varepsilon_{t + 1}^{\pi}(s) = & \sum_s \sum_{s_t} \mathbb P_{\pi}(s|s_t) \varepsilon_{t}^{\pi}(s_t) + \sum_s \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + \sum_{s_t}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \varepsilon_{t}^{\pi}(s_t) \right) \\
% = & \sum_{s_t} \varepsilon_{t}^{\pi}(s_t) + \widetilde{\mathcal O}\left( |\mathcal S|\sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + \sum_s\sum_{s_t}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \varepsilon_{t}^{\pi}(s_t) \right) \\
% %
% \leq & \sum_{s_t} \varepsilon_{t}^{\pi}(s_t) + \widetilde{\mathcal O}\left( |\mathcal S|\sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + |\mathcal S| \left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)|\right)
% \end{align}
\begin{align}
\sum_s |\varepsilon_{t + 1}^{\pi}(s)| \leq  & \sum_s \sum_{s_t} \mathbb P_{\pi}(s|s_t) |\varepsilon_{t}^{\pi}(s_t)| + \sum_s \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + \sum_{s_t}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) |\varepsilon_{t}^{\pi}(s_t)|\right) \\
%
\leq & \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| + \widetilde{\mathcal O}\left( |\mathcal S|\sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + |\mathcal S| \left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)|\right) \\
%
= & \left( 1 + \widetilde{\mathcal O} \left( |\mathcal S| \left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \right) \right) \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| + \widetilde{\mathcal O}\left( |\mathcal S|\sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \right)
\end{align}

Thus, we complete the proof.

\end{proof}

The proof of Theorem~\ref{thm:err_prop_2} is proved using the similar technique to that of Theorem~\ref{thm:err_prop_1}, but it also considers the self-normalization. The detailed proof is as follows.

\begin{proof}[Proof of Theorem \ref{thm:err_prop_2}]
% \end{proof}

Based on the idea of self-normalization, we have
\begin{align}
% \widehat d_{t}^{\pi}(s_t^i) = & d_{t}^{\pi}(s_t^i) + \varepsilon_{t}^{\pi}(s_t^i) \\
\widetilde d_{t + 1}^{\pi}(s_t^i) = & \frac{d_{t + 1}^{\pi}(s_{t + 1}^i) + \varepsilon_{t + 1}^{\pi}(s_{t + 1}^i)}{1 + \sum_{s} \varepsilon_{t + 1}^{\pi}(s_{t + 1}^i)},
\end{align}
where
\begin{align}
\varepsilon_{t + 1}^{\pi}(s) \coloneqq \frac{1}{n} \sum_{i = 1}^{n}\frac{\widetilde d_{t}^{\pi}(s_t^i)}{\widetilde d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) - d_{t + 1}^{\pi}(s).
\end{align}

Thus, we can analyze the self-normalized case using the similar method to the Proof of Theorem \ref{thm:err_prop_1}
\begin{align}
& d_{t + 1}^{\pi}(s) + \varepsilon_{t + 1}^{\pi}(s) \\
= & d_{t + 1}^{\pi}(s) + \sum_{s_t} \mathbb P_{\pi}(s|s_t) \widetilde \varepsilon_{t}^{\pi}(s_t) + \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \right) + \sum_{s_t} \widetilde{\mathcal O}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \widetilde \varepsilon_{t}^{\pi}(s_t)
\end{align}

Using the definition of $\varepsilon_{t + 1}^{\pi}(\cdot)$, we have
\begin{align}
\varepsilon_{t + 1}^{\pi}(s) =  & \sum_{s_t} \mathbb P_{\pi}(s|s_t) \widetilde\varepsilon_{t}^{\pi}(s_t) + \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + \sum_{s_t}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \widetilde \varepsilon_{t}^{\pi}(s_t)\right).
\end{align}

We first analyze $\sum_{s} \varepsilon_{t + 1}^{\pi}(s)$
\begin{align}
\sum_{s} \varepsilon_{t + 1}^{\pi}(s) = & \sum_s \sum_{s_t} \mathbb P_{\pi}(s|s_t) \widetilde \varepsilon_{t}^{\pi}(s_t) + \sum_s \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + \sum_{s_t}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \widetilde \varepsilon_{t}^{\pi}(s_t) \right) \\
= & \widetilde{\mathcal O}\left( |\mathcal S|\sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + \sum_s\sum_{s_t}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \widetilde \varepsilon_{t}^{\pi}(s_t) \right) \\
%
\leq & \widetilde{\mathcal O}\left( |\mathcal S|\sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + |\mathcal S| \left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)|\right)
\label{eq:normsumep}
\end{align}

We can obtain $\widetilde d_{t + 1}^{\pi}(s)$ satisfies the follows equality based on \eqref{eq:dhatnonnorm}
\begin{align}
\widetilde d_{t + 1}^{\pi}(s) = & \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \Bigg( d_{t + 1}^{\pi}(s) + \sum_{s_t} \mathbb P_{\pi}(s|s_t) \widetilde \varepsilon_{t}^{\pi}(s_t) \\
& + \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \right) + \sum_{s_t} \widetilde{\mathcal O}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \widetilde \varepsilon_{t}^{\pi}(s_t) \Bigg)
\end{align}

Based on the definition of $\varepsilon_{t + 1}^{\pi}(\cdot)$, we have
\begin{align}
\Rightarrow \widetilde \varepsilon_{t + 1}^{\pi}(s) = & \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \Bigg( d_{t + 1}^{\pi}(s) + \sum_{s_t} \mathbb P_{\pi}(s|s_t) \widetilde \varepsilon_{t}^{\pi}(s_t) \\
& + \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \right) + \sum_{s_t} \widetilde{\mathcal O}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \widetilde \varepsilon_{t}^{\pi}(s_t) \Bigg) - d_{t + 1}^{\pi}(s) \\
%
= & \left(-1 + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)}\right) d_{t + 1}^{\pi}(s) + \frac{\sum_{s_t} \mathbb P_{\pi}(s|s_t) \widetilde \varepsilon_{t}^{\pi}(s_t)}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \\
& + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \left( \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \right) + \sum_{s_t} \widetilde{\mathcal O}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \widetilde \varepsilon_{t}^{\pi}(s_t) \right) \\
%
\leq & \left(-1 + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)}\right) d_{t + 1}^{\pi}(s) + \frac{\sum_{s_t} \mathbb P_{\pi}(s|s_t) \widetilde \varepsilon_{t}^{\pi}(s_t)}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \\
& + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \left( \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + \left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)| \right) \right)
\end{align}

% We first consider $\sum_s \widetilde \varepsilon_{t + 1}^{\pi}(s)$
% \begin{align}
% \sum_s \widetilde \varepsilon_{t + 1}^{\pi}(s) \leq & \sum_s \left(-1 + \frac{1}{1 + \sum_s \varepsilon_t^\pi (s)}\right) d_{t + 1}^{\pi}(s) + \sum_s \frac{\sum_{s_t} \mathbb P_{\pi}(s|s_t) \varepsilon_{t}^{\pi}(s_t)}{1 + \sum_s \varepsilon_t^\pi (s)} \\
% %
% & + \frac{1}{1 + \sum_s \varepsilon_t^\pi (s)} \sum_s \left( \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + \left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| \right) \right) \\
% %
% = & -\frac{\sum_s \varepsilon_t^\pi (s)}{1 + \sum_s \varepsilon_t^\pi (s)} + \frac{\sum_s \varepsilon_t^\pi (s)}{1 + \sum_s \varepsilon_t^\pi (s)} \\
% & + \widetilde{\mathcal O}\left( \frac{|\mathcal S| \left(\sqrt{\max_{s}(w_t^2(s)) \eta^2} + \sqrt{ \eta^2} \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| \right)}{\sqrt{n} (1 + \sum_s \varepsilon_t^\pi (s))}  \right) \\
% % 
% = & \widetilde{\mathcal O}\left( \frac{|\mathcal S| \left(\sqrt{\max_{s}(w_t^2(s)) \eta^2} + \sqrt{ \eta^2} \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| \right)}{\sqrt{n} (1 + \sum_s \varepsilon_t^\pi (s))}  \right)
% \label{eq:normsumbound}
% \end{align}
% Thus, when $\sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| \leq 1$, it takes 
% \begin{align}
% H \asymp \frac{\sqrt{n}}{|\mathcal S| \left(\sqrt{\max_{s}(w_t^2(s)) \eta^2} + \sqrt{ \eta^2} \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| \right)}
% \end{align}
% before $\sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)|$ could reach $-0.5$.

We now discuss $\sum_s |\widetilde \varepsilon_{t + 1}^{\pi}(s)|$ based on the results above
\begin{align}
& \sum_s |\widetilde \varepsilon_{t + 1}^{\pi}(s)| \\
\leq & \sum_s \frac{|\sum_s \varepsilon_{t + 1}^\pi (s)|}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} d_{t + 1}^{\pi}(s) + \sum_s \frac{\sum_{s_t} \mathbb P_{\pi}(s|s_t) |\widetilde \varepsilon_{t}^{\pi}(s_t)|}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \\
& + \sum_s \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \left( \widetilde{\mathcal O}\left( \sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + \left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)| \right) \right) \\
%
= & \frac{\sum_s |\widetilde \varepsilon_t^\pi (s)|}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} + \frac{| \sum_s \varepsilon_{t + 1}^\pi (s)|}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \\
%
& + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \widetilde{\mathcal O}\left( |\mathcal S|\sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + |\mathcal S| \left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)|\right).
\end{align}

Then, substitute the results about $\sum_{s} \varepsilon_{t + 1}^{\pi}(s)$, \eqref{eq:normsumep}, into the last inequality, we have
\begin{align}
& \sum_s |\widetilde \varepsilon_{t + 1}^{\pi}(s)| \leq \\
& \frac{\sum_s |\widetilde \varepsilon_t^\pi (s)|}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \widetilde{\mathcal O}\left( |\mathcal S|\sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + |\mathcal S| \left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)|\right)\\
& + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \widetilde{\mathcal O}\left( |\mathcal S|\sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + |\mathcal S| \left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)|\right) \\
%
= & \frac{\sum_s |\widetilde \varepsilon_t^\pi (s)|}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \widetilde{\mathcal O}\left( |\mathcal S|\sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} + |\mathcal S| \left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)|\right) \\
= & \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \left( 1 + \widetilde{\mathcal O} \left( |\mathcal S|\sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{|\mathcal S|}{n\eta \eta_t} \right) \right) \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)|\\
& + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \widetilde{\mathcal O}\left( |\mathcal S|\sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \right),
\end{align}
where the $\sum_s \varepsilon_{t+ 1}^\pi (s)$ term in the denominator is defined in~\eqref{eq:normsumep}. This completes the proof.
% Thus our \textit{idea} is: choose unnormalized version if $(1 + \sum \varepsilon (s_t)) < 1$, otherwise choose the normalized version. Note that $(1 + \sum \varepsilon (s_t)) < 1 \iff \sum \tilde \pi (s_t) < 1$.

\end{proof}

Next, we provide the proof of corollary~\ref{cor:cor1}

\begin{proof}[Proof of Corollary~\ref{cor:cor1}]
Denote $x_t \coloneqq \sum_s |\widehat\varepsilon_{t + 1}^{\pi}(s)|$ for just this proof.
Under our assumption on a $\eta$, there is a universal constant $C$ such that 
$$
x_{t+1} \leq  (1+ \frac{C|\cS|}{\eta \sqrt{n}})x_{t}  +   \frac{C|\cS|}{\eta \sqrt{n}}.
$$
Note that $x_{0} \leq \frac{C|\cS|}{\eta \sqrt{n}}$. By the geometric series, the recursion implies that 
$$x_t\leq \sum_{i=0}^t  \frac{C|\cS|}{\eta \sqrt{n}} \left(1 + \frac{C|\cS|}{\eta \sqrt{n}}\right)^i =  \left(1 + \frac{C|\cS|}{\eta \sqrt{n}}\right)^t -1.$$

Under the assumption that $n$ is large, and $t\leq H$, we can further upper bound the above by 
$$
1 +  \frac{2C|\cS|}{\eta \sqrt{n}} - 1 = \frac{2C|\cS|}{\eta \sqrt{n}}.
$$
\end{proof}

==> sections/new_theory.tex <==
% !TEX root = ../neurips_2019.tex

\section{Theoretical Analysis for Recursive Estimator}

% For the moment, assume $\mu(s_t)$ is known.

% Let 
% \begin{align}
% \widetilde \pi(s_t) = & \pi(s_t) + \varepsilon(s_t) \\
% \widehat \pi(s_t) = & \frac{\pi(s_t) + \varepsilon(s_t)}{1 + \sum \varepsilon(s_t)},
% \end{align}
% where $\varepsilon(s_t)$ satisfies $\varepsilon(s_t) \geq -\pi(s_t)$ and $\sum \varepsilon(s_t) \geq -1$. Then,
% \begin{align}
% \widetilde \pi(s_{t+1}) = & \frac{1}{n} \sum_{i = 1}^{n}\frac{\widehat \pi(s_t^i)}{\mu(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s_{t+1}) \\
% = & \frac{1}{1 + \sum \varepsilon(s_t)} \left[ \frac{1}{n}\sum_{i = 1}^{n} \frac{\pi(s_t^i)}{\mu(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s_{t+1}) + \frac{1}{n}\sum_{i = 1}^{n} \frac{\varepsilon(s_t^i)}{\mu(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s_{t+1}) \right] \\
% = & \frac{1}{1 + \sum \varepsilon(s_t)} \Bigg[ \pi(s_{t+1}) + O\left( \frac{\sqrt{\mathbb E_{\mu} (\rho_t^2)}}{\sqrt{n}} \right) + \sum_{s_t} \underbrace{\frac{1}{n} \sum_{i = 1}^{n} \frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)} \mathbf 1(s_{t + 1}^i = s_{t + 1}, s_{t}^i = s_t)}_{= \mathbb P_{\pi}(s_{t+1}|s_t)\mu_{s_t} + O\left( \frac{\sqrt{\mathbb E_{\mu} [\rho_{t,a}^2]}}{\sqrt{n}} \right)} \frac{\varepsilon(s_t)}{\mu(s_t)} \Bigg] \\
% = & \frac{1}{1 + \sum \varepsilon(s_t)} \left[ \pi(s_{t+1}) + \sum_{s_t} \mathbb P_{\pi}(s_{t+1}|s_t) \varepsilon(s_t) + O\left( \frac{\sqrt{\mathbb E_{\mu} [\rho_{t}^2]}}{\sqrt{n}} + \frac{\sqrt{\max_{s_t} \mathbb E_{\mu} [\rho_{t,a}^2]} }{\sqrt{n}} \varepsilon(s_t) \right)\right].
% \end{align}
% Note that, the difference between normalized and unnormalized version is whether there is a $\frac{1}{1 + \sum \varepsilon(s_t)}$ term.

% We now discuss the $\varepsilon(s_t)$ term for the unnormalized case.
% \begin{align}
% \varepsilon(s_{t+1}) = & \sum_{s_t} \mathbb P_{\pi}(s_{t+1}|s_t)\varepsilon(s_t) + O\left( \frac{\sqrt{\mathbb E_{\mu} [\rho_{t}^2]}}{\sqrt{n}} + \frac{\sqrt{\max_{s_t} \mathbb E_{\mu} [\rho_{t,a}^2 | s_t]} }{\sqrt{n}} \sum_{s_t} \varepsilon(s_t) \right) \\
% |\varepsilon(s_{t+1})| \leq & \sum_{s_t} \mathbb P_{\pi}(s_{t+1}|s_t) |\varepsilon(s_t)| + O\left( \frac{\sqrt{\mathbb E_{\mu} [\rho_{t}^2]}}{\sqrt{n}} + \frac{\sqrt{\max_{s_t} \mathbb E_{\mu} [\rho_{t,a}^2 | s_t]} }{\sqrt{n}} \sum_{s_t} |\varepsilon(s_t)| \right).
% \end{align}
% Take summation over $s_{t+1}$ on both sides, we have the following results for the unnormalized version,
% \begin{align}
% \sum_{s_{t+1}}|\varepsilon(s_{t+1})| \leq & \sum_{s_{t}} |\varepsilon(s_{t})| + O\left( \frac{|\mathcal S|\sqrt{\mathbb E_{\mu} [\rho_{t}^2]}}{\sqrt{n}} + \frac{|\mathcal S|\sqrt{\max_{s_t} \mathbb E_{\mu} [\rho_{t,a}^2 | s_t]} }{\sqrt{n}} \sum_{s_t} |\varepsilon(s_{t})| \right) \\
% \Rightarrow \sum_{s_{t+1}}|\varepsilon(s_{t+1})| \leq & \left( 1 + O\left(\frac{|\mathcal S|\sqrt{\max_{s_t} \mathbb E_{\mu} [\rho_{t,a}^2 | s_t]} }{\sqrt{n}} \right) \right)\sum_{s_{t}}|\varepsilon(s_{t})| + \frac{\sqrt{\mathbb E_{\mu} [\rho_{t}^2]}}{\sqrt{n}}.
% \end{align}
% %
% %\note[tx]{I modified a little for the (in)equation above}
% %
% Thus, if $\sum_{s_{t}} |\varepsilon(s_{t})| \leq 1$, the error grows linearly; and if $\sum_{s_{t}}|\varepsilon(s_{t})| > 1$, the error grows exponentially but with a small factor. Since that, we can handle horizon up to $H = {\sqrt{n}}/{\sqrt{\mathbb{E} [\rho_t^2]}}$.

% For the case with normalization, $\varepsilon(s_{t+1})$ becomes different
% \begin{align}
% \varepsilon(s_{t+1}) = & -\pi(s_{t+1}) + \frac{1}{n} \sum_{i = 1}^{n}\frac{\widehat \pi(s_t^i)}{\mu(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s_{t+1}) \\
% = & -\pi(s_{t+1}) + \frac{1}{1 + \sum \varepsilon (s_t)} \left( \pi(s_{t+1}) + O\left( \frac{\sqrt{\mathbb E [\rho_t^2]}}{\sqrt{n}} \right) \right) \\
% & + \frac{1}{1 + \sum \varepsilon (s_t)} \left( \sum_{s_t} \mathbb P_{\pi}(s_{t+1}|s_t)\varepsilon(s_t) + O\left( \frac{\sqrt{\mathbb E_{\mu}[\rho_{t,a}^2]}}{\sqrt{n}} |\varepsilon (s_t)| \right) \right) \\
% = & \left(-1 + \frac{1}{1 + \sum \varepsilon (s_t)}\right) \pi(s_{t+1}) + \frac{\sum_{s_t}P_{\pi}(s_{t+1}|s_t)\varepsilon(s_t)}{1 + \sum \varepsilon (s_t)} \\
% & + \frac{1}{1 + \sum \varepsilon (s_t)} O\left( \frac{\sqrt{\mathbb E_{\mu}[\rho_{t}^2]}}{\sqrt{n}} + \frac{\sqrt{\mathbb E_{\mu}[\rho_{t,a}^2]}}{\sqrt{n}} |\varepsilon (s_t)|\right).
% \end{align}
% Let's first calculate $\sum_{s_{t+1}} \varepsilon (s_{t+1})$
% \begin{align}
% \sum_{s_{t+1}} \varepsilon (s_{t+1}) = -\frac{\sum \varepsilon(s_t)}{1 + \sum \varepsilon(s_t)} + \frac{\sum \varepsilon(s_t)}{1 + \sum \varepsilon(s_t)} + O\left( \frac{|\mathcal S_{t+1}| \left(\sqrt{\mathbb E_{\mu}[\rho_{t}^2]} + \sqrt{\mathbb E_{\mu}[\rho_{t,a}^2]} |\varepsilon (s_t)| \right)}{\sqrt{n} (1 + \sum \varepsilon (s_t))}  \right).
% \end{align}
% Thus, when $|\varepsilon(s_t)| \leq 1$, it takes 
% \begin{align}
% H \asymp \frac{\sqrt{n}}{|\mathcal S| \left(\sqrt{\mathbb E_{\mu}[\rho_{t}^2]} + \sqrt{\mathbb E_{\mu}[\rho_{t,a}^2]} |\varepsilon (s_t)| \right)}
% \end{align}
% before $\sum_{s_{t+1}}\varepsilon(s_{t+1})$ could reach $-0.5$.

% Now
% \begin{align}
% \|\varepsilon(s_{t+1})\|_1 \leq \frac{\|\varepsilon(s_t)\|_1}{1 + \sum \varepsilon(s_t)} + \frac{|\mathcal S_{t+1}||\sum_{s_t}\varepsilon(s_t)|}{1 + \sum \varepsilon(s_t)} + O \left( \frac{ |\mathcal S_{t+1}| \left(\sqrt{\mathbb E_{\mu}[\rho_{t}^2]} + \sqrt{\mathbb E_{\mu}[\rho_{t,a}^2]} |\varepsilon (s_t)| \right)}{\sqrt{n} (1 + \sum \varepsilon (s_t))} \right).
% \end{align}

% Collecting the bounds we get:
% \begin{align}
% |\varepsilon(s_{t+1})| \leq & \left( \frac{1 + \frac{|\mathcal S_{t+1}|\sqrt{ \mathbb E_{\mu}[\rho_{t,a}^2]}}{\sqrt{n}}}{1 + \sum \varepsilon (s_t)} \right) |\varepsilon(s_{t})| + \frac{|\mathcal S_{t+1}|^2 \sqrt{\mathbb E_{\mu}[\rho_{t}^2]}}{\sqrt{n} (1 + \sum \varepsilon (s_t))^2} \\
% & +  \frac{|\mathcal S_{t+1}|^2 \sqrt{\mathbb E_{\mu}[\rho_{t,a}^2]}}{\sqrt{n} (1 + \sum \varepsilon (s_t)))^2} |\varepsilon(s_t)| + \frac{|\mathcal S_{t+1}| \sqrt{\mathbb E_{\mu}[\rho_{t}^2]}}{\sqrt{n} (1 + \sum \varepsilon (s_t))}
% \end{align}

% This is quantitatively the same as the version without normalization. But it strictly reduces the error if $(1 + \sum \varepsilon (s_t)) > 1$.

% Thus our \textit{idea} is: choose unnormalized version if $(1 + \sum \varepsilon (s_t)) < 1$, otherwise choose the normalized version. Note that $(1 + \sum \varepsilon (s_t)) < 1 \iff \sum \tilde \pi (s_t) < 1$.


% \subsection{Full version}

\begin{proof}[Proof of Theorem \ref{thm:err_prop_1}]

% \paragraph{Non-normalized case:}

\note[Tengyang]{Give $d_\mu$ a minimal value, as $\eta$}

Given the definition of the non-normalized estimation $\widehat d_{t}^{\pi}(s_t^i)$ in \eqref{eq:dpirecest1}, we have
\begin{align}
& \widehat d_{t + 1}^{\pi}(s) \\
= & \frac{1}{n} \sum_{i = 1}^{n}\frac{\widehat d_{t}^{\pi}(s_t^i)}{\widehat d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \\
= & \frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i) + \varepsilon_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i) + \varepsilon_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \\
= & \frac{1}{n} \sum_{i = 1}^{n} \left(\frac{(d_{t}^{\pi}(s_t^i) + \varepsilon_{t}^{\pi}(s_t^i)) (d_{t}^{\mu}(s_t^i) - \varepsilon_{t}^{\mu}(s_t^i))}{(d_{t}^{\mu}(s_t^i))^2 - (\varepsilon_{t}^{\mu}(s_t^i))^2} \right) \frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \\
= & \frac{1}{n} \sum_{i = 1}^{n} \left(\frac{(d_{t}^{\pi}(s_t^i) + \varepsilon_{t}^{\pi}(s_t^i)) (d_{t}^{\mu}(s_t^i) - \varepsilon_{t}^{\mu}(s_t^i))}{(d_{t}^{\mu}(s_t^i))^2} + \frac{d_{t}^{\pi}(s_t^i)}{(d_{t}^{\mu}(s_t^i))^3} \widetilde{\mathcal O}\left( \frac{1}{n} \right) \right) \frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \\
%
%
%
= & \underbrace{\frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \left(1 + \widetilde{\mathcal O}\left( \frac{1}{n}\right)\right)}_{\text{(a)}} + \underbrace{\frac{1}{n} \sum_{i = 1}^{n}\frac{\varepsilon_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s)}_{\text{(b)}} \\
& + \underbrace{\frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i) \varepsilon_{t}^{\mu}(s_t^i)}{(d_{t}^{\mu}(s_t^i))^2}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s)}_{\text{(c)}} + \underbrace{\frac{1}{n} \sum_{i = 1}^{n}\frac{\varepsilon_{t}^{\pi}(s_t^i) \varepsilon_{t}^{\mu}(s_t^i)}{(d_{t}^{\mu}(s_t^i))^2}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s)}_{\text{(d)}}.
\end{align}

We now analyze these four terms above separately. For the term (a):
\begin{align}
& \frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \left(1 + \widetilde{\mathcal O}\left( \frac{1}{n}\right)\right) \\
= & \left( d_{t + 1}^{\pi}(s) + \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} \right) \right)  \left(1 + \widetilde{\mathcal O}\left( \frac{1}{n}\right)\right) \\
= & d_{t + 1}^{\pi}(s) + \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} \right)
\label{eq:terma}
\end{align}

For the term (b):
\begin{align}
& \frac{1}{n} \sum_{i = 1}^{n}\frac{\varepsilon_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \\
= & \sum_{s_t}\frac{1}{n} \sum_{i = 1}^{n}\frac{\pi(a_t^i|s_t)}{\mu(a_t^i|s_t)}\mathbf 1(s_{t}^i = s_t, s_{t+1}^i = s) \frac{\varepsilon_{t}^{\pi}(s_t)}{d_{t}^{\mu}(s_t)} \\
= & \sum_{s_t} d_{t}^{\mu}(s_t) \left[ \mathbb P_{\pi}(s|s_t) + \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} \right)\right] \frac{\varepsilon_{t}^{\pi}(s_t)}{d_{t}^{\mu}(s_t)} \\
= & \sum_{s_t} \left[ \mathbb P_{\pi}(s|s_t) + \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} \right) \right] \varepsilon_{t}^{\pi}(s_t)
\label{eq:termb}
\end{align}

For the term (c):
\begin{align}
& \frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i) \varepsilon_{t}^{\mu}(s_t^i)}{(d_{t}^{\mu}(s_t^i))^2}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \\
= & \frac{1}{n} \sum_{i = 1}^{n}\frac{d_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \frac{\varepsilon_{t}^{\mu}(s_t^i)}{d_{t}^{\mu}(s_t^i)} \\
= & \left( d_{t + 1}^{\pi}(s) + \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} \right) \right) \frac{\widetilde{\mathcal O}\left( \frac{1}{\sqrt{n}} \right)}{d_{t}^{\mu}(s_t^i)}
\label{eq:termc}
\end{align}

For the term (d):
\begin{align}
& \frac{1}{n} \sum_{i = 1}^{n}\frac{\varepsilon_{t}^{\pi}(s_t^i) \varepsilon_{t}^{\mu}(s_t^i)}{(d_{t}^{\mu}(s_t^i))^2}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \\
= & \frac{1}{n} \sum_{i = 1}^{n}\frac{\varepsilon_{t}^{\pi}(s_t^i)}{d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) \frac{\varepsilon_{t}^{\mu}(s_t^i)}{d_{t}^{\mu}(s_t^i)} \\
= & \sum_{s_t} \left[ \mathbb P_{\pi}(s|s_t) + \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]  }{n}} \right)\right] \frac{\varepsilon_{t}^{\pi}(s_t) \widetilde{\mathcal O}\left( \frac{1}{\sqrt{n}} \right)}{d_{t}^{\mu}(s_t^i)}
\label{eq:termd}
\end{align}

Combining \eqref{eq:terma}, \eqref{eq:termb}, \eqref{eq:termc} and \eqref{eq:termd}, we obtain
\begin{align}
\widehat d_{t + 1}^{\pi}(s) = & d_{t + 1}^{\pi}(s) + \sum_{s_t} \mathbb P_{\pi}(s|s_t) \varepsilon_{t}^{\pi}(s_t) + \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} \right) + \sum_{s_t} \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]  }{n}} \right) \varepsilon_{t}^{\pi}(s_t) \\
\end{align}
\begin{align}
\Rightarrow \varepsilon_{t + 1}^{\pi}(s) =  & \sum_{s_t} \mathbb P_{\pi}(s|s_t) \varepsilon_{t}^{\pi}(s_t) + \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + \sum_{s_t}\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} \varepsilon_{t}^{\pi}(s_t)\right) \\
%
\sum_{s} \varepsilon_{t + 1}^{\pi}(s) = & \sum_s \sum_{s_t} \mathbb P_{\pi}(s|s_t) \varepsilon_{t}^{\pi}(s_t) + \sum_s \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + \sum_{s_t}\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} \varepsilon_{t}^{\pi}(s_t) \right) \\
= & \sum_{s_t} \varepsilon_{t}^{\pi}(s_t) + \mathcal O_p\left( |\mathcal S|\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + \sum_s\sum_{s_t}\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} \varepsilon_{t}^{\pi}(s_t) \right) \\
%
\leq & \sum_{s_t} \varepsilon_{t}^{\pi}(s_t) + \mathcal O_p\left( |\mathcal S|\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + |\mathcal S| \sqrt{\frac{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)|\right)
\end{align}
\begin{align}
|\varepsilon_{t + 1}^{\pi}(s)| \leq  & \sum_{s_t} \mathbb P_{\pi}(s|s_t) |\varepsilon_{t}^{\pi}(s_t)| + \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + \sum_{s_t}\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} |\varepsilon_{t}^{\pi}(s_t)|\right) \\
%
\sum_s |\varepsilon_{t + 1}^{\pi}(s)| \leq  & \sum_s \sum_{s_t} \mathbb P_{\pi}(s|s_t) |\varepsilon_{t}^{\pi}(s_t)| + \sum_s \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + \sum_{s_t}\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} |\varepsilon_{t}^{\pi}(s_t)|\right) \\
%
\leq & \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| + \mathcal O_p\left( |\mathcal S|\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + |\mathcal S| \sqrt{\frac{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)|\right) \\
%
= & \left( 1 + \mathcal O_p \left( |\mathcal S| \sqrt{\frac{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} \right) \right) \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| + \mathcal O_p\left( |\mathcal S|\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} \right)
\end{align}
\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:err_prop_2}]
% \end{proof}

Based on the idea of self-normalization, we have
\begin{align}
% \widehat d_{t}^{\pi}(s_t^i) = & d_{t}^{\pi}(s_t^i) + \varepsilon_{t}^{\pi}(s_t^i) \\
\widetilde d_{t + 1}^{\pi}(s_t^i) = & \frac{d_{t + 1}^{\pi}(s_{t + 1}^i) + \varepsilon_{t + 1}^{\pi}(s_{t + 1}^i)}{1 + \sum_{s} \varepsilon_{t + 1}^{\pi}(s_{t + 1}^i)},
\end{align}
where
\begin{align}
\varepsilon_{t + 1}^{\pi}(s) \coloneqq \frac{1}{n} \sum_{i = 1}^{n}\frac{\widetilde d_{t}^{\pi}(s_t^i)}{\widetilde d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) - d_{t + 1}^{\pi}(s).
\end{align}

Thus, we can analyze the self-normalized case similarly as follows
\begin{align}
d_{t + 1}^{\pi}(s) + \varepsilon_{t + 1}^{\pi}(s) = & d_{t + 1}^{\pi}(s) + \sum_{s_t} \mathbb P_{\pi}(s|s_t) \widetilde \varepsilon_{t}^{\pi}(s_t) + \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} \right) + \sum_{s_t} \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]  }{n}} \right) \widetilde \varepsilon_{t}^{\pi}(s_t)
\end{align}
\begin{align}
\Rightarrow \varepsilon_{t + 1}^{\pi}(s) =  & \sum_{s_t} \mathbb P_{\pi}(s|s_t) \widetilde\varepsilon_{t}^{\pi}(s_t) + \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + \sum_{s_t}\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} \widetilde \varepsilon_{t}^{\pi}(s_t)\right) \\
%
\sum_{s} \varepsilon_{t + 1}^{\pi}(s) = & \sum_s \sum_{s_t} \mathbb P_{\pi}(s|s_t) \widetilde \varepsilon_{t}^{\pi}(s_t) + \sum_s \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + \sum_{s_t}\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} \widetilde \varepsilon_{t}^{\pi}(s_t) \right) \\
= & \mathcal O_p\left( |\mathcal S|\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + \sum_s\sum_{s_t}\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} \widetilde \varepsilon_{t}^{\pi}(s_t) \right) \\
%
\leq & \mathcal O_p\left( |\mathcal S|\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + |\mathcal S| \sqrt{\frac{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)|\right)
\end{align}
\begin{align}
\Rightarrow \widetilde d_{t + 1}^{\pi}(s) = & \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \Bigg( d_{t + 1}^{\pi}(s) + \sum_{s_t} \mathbb P_{\pi}(s|s_t) \widetilde \varepsilon_{t}^{\pi}(s_t) \\
& + \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} \right) + \sum_{s_t} \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]  }{n}} \right) \widetilde \varepsilon_{t}^{\pi}(s_t) \Bigg)
\end{align}
\begin{align}
\Rightarrow \widetilde \varepsilon_{t + 1}^{\pi}(s) = & \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \Bigg( d_{t + 1}^{\pi}(s) + \sum_{s_t} \mathbb P_{\pi}(s|s_t) \widetilde \varepsilon_{t}^{\pi}(s_t) \\
& + \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} \right) + \sum_{s_t} \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]  }{n}} \right) \widetilde \varepsilon_{t}^{\pi}(s_t) \Bigg) - d_{t + 1}^{\pi}(s) \\
%
= & \left(-1 + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)}\right) d_{t + 1}^{\pi}(s) + \frac{\sum_{s_t} \mathbb P_{\pi}(s|s_t) \widetilde \varepsilon_{t}^{\pi}(s_t)}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \\
& + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \left( \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} \right) + \sum_{s_t} \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]  }{n}} \right) \widetilde \varepsilon_{t}^{\pi}(s_t) \right) \\
%
\leq & \left(-1 + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)}\right) d_{t + 1}^{\pi}(s) + \frac{\sum_{s_t} \mathbb P_{\pi}(s|s_t) \widetilde \varepsilon_{t}^{\pi}(s_t)}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \\
& + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \left( \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + \sqrt{\frac{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]  }{n}} \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)| \right) \right)
\end{align}

% We first consider $\sum_s \widetilde \varepsilon_{t + 1}^{\pi}(s)$
% \begin{align}
% \sum_s \widetilde \varepsilon_{t + 1}^{\pi}(s) \leq & \sum_s \left(-1 + \frac{1}{1 + \sum_s \varepsilon_t^\pi (s)}\right) d_{t + 1}^{\pi}(s) + \sum_s \frac{\sum_{s_t} \mathbb P_{\pi}(s|s_t) \varepsilon_{t}^{\pi}(s_t)}{1 + \sum_s \varepsilon_t^\pi (s)} \\
% %
% & + \frac{1}{1 + \sum_s \varepsilon_t^\pi (s)} \sum_s \left( \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + \sqrt{\frac{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]  }{n}} \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| \right) \right) \\
% %
% = & -\frac{\sum_s \varepsilon_t^\pi (s)}{1 + \sum_s \varepsilon_t^\pi (s)} + \frac{\sum_s \varepsilon_t^\pi (s)}{1 + \sum_s \varepsilon_t^\pi (s)} \\
% & + \mathcal O_p\left( \frac{|\mathcal S| \left(\sqrt{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]} + \sqrt{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]} \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| \right)}{\sqrt{n} (1 + \sum_s \varepsilon_t^\pi (s))}  \right) \\
% % 
% = & \mathcal O_p\left( \frac{|\mathcal S| \left(\sqrt{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]} + \sqrt{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]} \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| \right)}{\sqrt{n} (1 + \sum_s \varepsilon_t^\pi (s))}  \right)
% \label{eq:normsumbound}
% \end{align}
% Thus, when $\sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| \leq 1$, it takes 
% \begin{align}
% H \asymp \frac{\sqrt{n}}{|\mathcal S| \left(\sqrt{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]} + \sqrt{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]} \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| \right)}
% \end{align}
% before $\sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)|$ could reach $-0.5$.

We now discuss $\sum_s |\widetilde \varepsilon_{t + 1}^{\pi}(s)|$
\begin{align}
\sum_s |\widetilde \varepsilon_{t + 1}^{\pi}(s)| \leq & \sum_s \frac{|\sum_s \varepsilon_{t + 1}^\pi (s)|}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} d_{t + 1}^{\pi}(s) + \sum_s \frac{\sum_{s_t} \mathbb P_{\pi}(s|s_t) |\widetilde \varepsilon_{t}^{\pi}(s_t)|}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \\
& + \sum_s \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \left( \mathcal O_p\left( \sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + \sqrt{\frac{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]  }{n}} \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)| \right) \right) \\
%
= & \frac{\sum_s |\widetilde \varepsilon_t^\pi (s)|}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} + \underbrace{\frac{| \sum_s \varepsilon_{t + 1}^\pi (s)|}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)}}_{\text(a)} \\
%
& + \mathcal O_p\left( \frac{ |\mathcal S| \sqrt{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]} + |\mathcal S| \sqrt{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]} \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)|}{\sqrt{n} (1 + \sum_s \varepsilon_{t + 1}^\pi (s))} \right).
\end{align}
% Substitute the bound \eqref{eq:normsumbound} into term (a), we obtain
\begin{align}
& \sum_s |\widetilde \varepsilon_{t + 1}^{\pi}(s)| \\
\leq & \frac{\sum_s |\widetilde \varepsilon_t^\pi (s)|}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \mathcal O_p\left( |\mathcal S|\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} + |\mathcal S| \sqrt{\frac{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)|\right)\\
%
& + \mathcal O_p\left( \frac{|\mathcal S| \left(\sqrt{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]} + \sqrt{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]} \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)| \right)}{\sqrt{n} (1 + \sum_s \varepsilon_{t + 1}^\pi (s)) } \right) \\
= & \frac{\sum_s |\widetilde \varepsilon_t^\pi (s)|}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} + \mathcal O_p\left( \frac{|\mathcal S| \left(\sqrt{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]} + \sqrt{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t ]} \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)| \right)}{\sqrt{n} (1 + \sum_s \varepsilon_{t + 1}^\pi (s)) } \right) \\
= & \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \left( 1 + \mathcal O_p \left( |\mathcal S| \sqrt{\frac{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }{n}} \right) \right) \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)| + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \mathcal O_p\left( |\mathcal S|\sqrt{\frac{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }{n}} \right).
\end{align}
% Thus our \textit{idea} is: choose unnormalized version if $(1 + \sum \varepsilon (s_t)) < 1$, otherwise choose the normalized version. Note that $(1 + \sum \varepsilon (s_t)) < 1 \iff \sum \tilde \pi (s_t) < 1$.

\end{proof}

==> sections/ratio_est.tex <==
% !TEX root = ../neurips_2019.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Marginalized Density Ratio Estimation and OPE}
\label{sec:estratio}


In this section, we present our estimators for $w_t(\cdot)$ which is defined by the marginalized ratio $d_t^{\pi}(\cdot) / d_t^{\mu}(\cdot)$ at time step $t$. Since the initial state distribution $d_0(\cdot)$ and the marginalized state distribution of behavior policy $d_t^{\mu}(\cdot)$ are the same as the data distribution, which allows us to obtain the on-policy estimation for $d_0(\cdot)$ and $d_t^{\mu}(\cdot)$ directly, we will focus on the estimate of $d_t^{\pi}(\cdot)$ in this section. In the following parts, we use $(s_t,a_t) \sim d_t^{\pi}$ to denote drawing from distribution $d_t^{\pi}(s_t,a_t) \coloneqq d_t^{\pi}(s_t) \pi(a_t|s_t)$, and we also use $(s_t,a_t) \sim d_t^{\mu}$ similarly. We define $T_t^{\pi}(s'|s) \coloneqq \sum_{a} \pi(a|s) T_t^{\pi}(s'|s,a)$ as the state transition probability from $s$ to $s'$ at time step $t$ under policy $\pi$.

Our idea to estimate $d_t^{\pi}(\cdot)$ is to use the relationship between $d_t^{\pi}(\cdot)$ and $d_{t + 1}^{\pi}(\cdot)$ to optimize the data efficiency. Given the definition of $T_t^{\pi}(s'|s)$, we have $d_{t + 1}^{\pi}(\cdot)$ is satisfying
\begin{align}
d_t^{\pi}(s_{t + 1}) = & \mathbb E_{s_t \sim d_t^{\pi}} \left[T_t^{\pi}(s_{t + 1} | s_t) \right]\\
= & \mathbb E_{(s_t,a_t) \sim d_t^{\pi}} \left[ T_t(s_{t + 1} | s_t,a_t) \right] \\
= & \mathbb E_{(s_t,a_t) \sim d_t^{\mu}} \left[ \frac{d_t^{\pi}(s_{t})}{d_t^{\mu}(s_{t})} \frac{\pi(a_t|s_t)}{\mu(a_t|s_t)}  T_t(s_{t + 1} | s_t,a_t) \right].
\end{align}
The equality above can be leveraged to estimate $d_{t}^{\pi}(\cdot)$ recursively. Note that we have $d_{0}^{\mu}(\cdot) = d_{0}^{\mu}(\cdot) = d_0 (\cdot)$, and then our first estimator for $d_{t}^{\pi}(\cdot)$ is as follows
\begin{align}
\widehat d_{t + 1}^{\pi}(s) = & \frac{1}{n} \sum_{i = 1}^{n}\frac{\widehat d_{t}^{\pi}(s_t^i)}{\widehat d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s).
\label{eq:dpirecest1}
\end{align}

Since $d_{t}^{\pi}(\cdot)$ always satisfies the normalization property (i.e. $\sum_{s \in \mathcal S} d_{t}^{\pi}(s) = 1$), we can obtain another estimator of $d_{t}^{\pi}(\cdot)$ using self-normalization as follows
\begin{align}
\widetilde d_{t + 1}^{\pi}(s) = \frac{\sum_{i = 1}^{n}\frac{\widehat d_{t}^{\pi}(s_t^i)}{\widehat d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s)}{\sum_{i = 1}^{n}\frac{\widehat d_{t}^{\pi}(s_t^i)}{\widehat d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)}}.
\label{eq:dpirecest2}
\end{align}

\note[ym]{ Do we need an Algorithm to summarize the recursive estimators?} \note[tx]{Let me summarize it (please edit directly if you feel anything not good enough)}


Estimators~\eqref{eq:dpirecest1} and~\eqref{eq:dpirecest2} above provide the off-policy estimate of $\widehat d_t^{\pi}(\cdot)$,
which can then be plugged in to \eqref{eq:w-and-v} to estimate $\widehat w_{t}(s)=\nicefrac{\widehat d_{t}^\pi(s)}{\widehat d_{t}^\mu(s)}$ recursively and $\widehat v(\pi)$ eventually.
Notice, the state distributions induced by the behavior policies can be obtained via direct counting $\widehat d_t^{\mu}(s) = \frac{1}{n}\sum_{i = 1}^{n} \mathbf{1}(s_t^i = s)$.
Further, when the MDPs induced by the behavior policies have small mixing diameters, the $\widehat d_t^\mu$ can be estimated rather accurately. Algorithm~\ref{alg:mainalgo} in Appendix~\ref{app:alg} shows the complete DAG-MDP estimators in pseudo codes.


% Note that, our estimators of $d_{t + 1}^{\pi}(\cdot)$ leverage the estimation of $d_{t}^{\pi}(\cdot)$, and thus, we obtain the estimate of $d_t^{\pi}(\cdot)$ recursively. The estimation of $d_0(\cdot)$ and $d_t^{\mu}(\cdot)$ can be obtained directed by using the on-policy data ($\widehat d_0(s) = \frac{1}{n}\sum_{i = 1}^{n} \mathbf{1}(s_0^i == s)$ and $\widehat d_t^{\mu}(s) = \frac{1}{n}\sum_{i = 1}^{n} \mathbf{1}(s_t^i == s)$). Since that, we can calculate the estimators of marginalized density ratio according to its definition $w_t(s) = d_t^{\pi}(s) / d_t^{\mu}(s)$.  


% Thus, we have the recursive off-policy estimation for $d_t^{\pi}(\cdot)$, which leverages the marginalized distribution of previous time step to achieve better data-efficiency. Combining with the on-policy estimation for $d_0(\cdot)$ and $d_t^{\mu}(\cdot)$ ($\widehat d_0(s) = \frac{1}{n}\sum_{i = 1}^{n} \mathbf{1}(s_0^i == s)$ and $\widehat d_t^{\mu}(s) = \frac{1}{n}\sum_{i = 1}^{n} \mathbf{1}(s_t^i == s)$), we obtain the estimators of marginalized density ratio, denoting $\widehat w_t(\cdot)$ or $\widetilde w_t(\cdot)$ separately if we use~\eqref{eq:dpirecest1} or~\eqref{eq:dpirecest2} as the numerator.


\subsection{Theoretical Analysis}

In this section, we provide a theoretical analysis of our estimators of $w_t(\cdot)$. We study the error propagation of our recursive estimators. Our theoretical results show that the dependence of our recursive estimators is polynomial on the horizon. This is in contrast to the Tree-IS estimators, which may have exponential dependencies. Example~\ref{ex:IS-exponential} shows one case of the exponential dependencies of the Tree-IS estimators.

% \note[ym]{ The main message is to show that the dependence is polynomial on the horizon. This is in contrast to the IS-based estimators, which may have exponential dependencies (see Example~\ref{ex:IS-exponential}).}
\begin{example}
\label{ex:IS-exponential}
Vanilla Tree-IS weights are products of single-step IS weights, i.e.,
$\log\rho_{0:H}=\sum_{t=0}^{H-1}\log\rho_{t}$.
Let $E_{\log}=\mathbb{E}\log\rho_{t}$ and $V_{\log}=\mathbb{V}\log\rho_{t}$ be the mean and variance of the single-step log-IS weights and, for simplicity, suppose the policies are iid at different times.
By Central Limit Theorem, $\log\rho_{0:H}$ asymptotically follows a normal distribution with parameters $\bigl(-HE_{\log}, HV_{\log}\bigr)$.
As a result,
the Tree-IS weights asymptotically follow a log-normal distribution with variance
$\bigl(\exp\bigl(HV_{\log}\bigr)-1\bigr)$, which is exponential in the horizon $H$.
\end{example}

We first consider $\widehat d_{0}(\cdot)$ and $\widehat d_{t}^{\mu}(\cdot)$, since we can use on-policy data to estimate these distributions. Hoeffding's inequality implies the following fact.

\begin{fact}
\label{fct:fct1}
For $\widehat d_{0}(s)$ and $\widehat d_{t}^{\mu}(s_t^i)$, $\forall s \in \mathcal S$, w.p. $1 - \delta$, we have
\begin{align}
\widehat d_{0}(s) = d_{0}(s) + \varepsilon_0(s) = d_{0}(s) + \widetilde{\mathcal O}\left( \frac{1}{\sqrt{n}} \right) \\
\widehat d_{t}^\mu(s) = d_{t}^\mu(s) + \varepsilon_{t}^\mu(s) = d_{t}^\mu(s) + \widetilde{\mathcal O}\left( \frac{1}{\sqrt{n}} \right).
\end{align}
%by using Hoeffding's inequality.
\end{fact}

\paragraph{Error propagation}

We now discuss the error propagation of our first recursive estimator for $d_{t}^{\pi}(\cdot)$ (defined in~\eqref{eq:dpirecest1}). Over this section, we assume there exists a $\eta > 0$, such that $\pi(a|s) / \mu(a|s) \leq 1 / \eta$ for any $(s,a)$. We also assume there exists $\{\eta_t > 0\}_{t = 0}^{H - 1}$, such that $d_t^{\mu}(s) \geq \eta_t$ for all $s$ and $t$. Thus, we have theorems for error propagation as follows. 

% \note[tx]{I used $\pi(a|s) / \mu(a/s) \leq \eta$ below}
\begin{theorem}
\label{thm:err_prop_1}
Let $\widehat d_t^{\pi}(\cdot)$ be the estimator of $d_{t}^{\pi}(\cdot)$, defined in~\eqref{eq:dpirecest1}. Let $\widehat \varepsilon_t^{\pi}(s) \coloneqq \widehat d_t^{\pi}(s) - d_t^{\pi}(s)$, then we have
% \begin{align}
% & \sum_s |\widehat\varepsilon_{t + 1}^{\pi}(s)| \\
% \leq & \left( 1 + \mathcal O_p \left( |\mathcal S| \frac{\sqrt{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }}{\sqrt{n}} \right) \right) \sum_{s_t} |\widehat\varepsilon_{t}^{\pi}(s_t)| \\
% & + \mathcal O_p\left( |\mathcal S|\frac{\sqrt{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }}{\sqrt{n}} \right).
% \end{align}
\begin{align}
& \sum_s |\widehat\varepsilon_{t + 1}^{\pi}(s)| 
% \\
\leq 
% & 
\left( 1 + \widetilde{\mathcal O} \left( |\mathcal S| \sqrt{\frac{\eta^2 }{n}} \right) \right) \sum_{s_t} |\varepsilon_{t}^{\pi}(s_t)| \\
&\hspace{4em} + \widetilde{\mathcal O}\left( |\mathcal S|\sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \right).
\end{align}
\end{theorem}
We provide the detailed proof of Theorem~\eqref{thm:err_prop_1} in Appendix~\ref{app:proof_sec4}. Theorem~\ref{thm:err_prop_1} provides the properties of error propagation for the recursive estimator~\eqref{eq:dpirecest1}. It implies that $\sum_s |\widehat\varepsilon_{t + 1}^{\pi}(s)|$ only has polynomial dependence on the horizon if $n$ is large enough. We discuss this dependence later in this section.


The error propagation for the recursive estimator~\eqref{eq:dpirecest2} is as follows
\begin{theorem}
\label{thm:err_prop_2}
Let $\widetilde d_t^{\pi}(\cdot)$ be the estimator of $d_{t}^{\pi}(\cdot)$, defined in~\eqref{eq:dpirecest2}. Let $\widetilde \varepsilon_t^{\pi}(s) \coloneqq \widetilde d_t^{\pi}(s) - d_t^{\pi}(s)$, and $\varepsilon_{t + 1}^{\pi}(s) \coloneqq \frac{1}{n} \sum_{i = 1}^{n}\frac{\widetilde d_{t}^{\pi}(s_t^i)}{\widetilde d_{t}^{\mu}(s_t^i)}\frac{\pi(a_t^i|s_t^i)}{\mu(a_t^i|s_t^i)} \mathbf 1(s_{t+1}^i = s) - d_{t + 1}^{\pi}(s)$, then we have
% \begin{align}
% & \sum_s |\widetilde \varepsilon_{t + 1}^{\pi}(s)| \\
% \leq & \frac{\left( 1 + \mathcal O_p \left( |\mathcal S| \frac{\sqrt{\max_{s_t} \mathbb E_{\mu}[\rho_t^2(s_t,a_t) | s_t]  }}{\sqrt{n}} \right) \right) \sum_{s_t} |\widetilde \varepsilon_{t + 1}^{\pi}(s_t)|}{(1 + \sum_{s} \varepsilon_{t + 1}^{\pi}(s))} \\
% & + \mathcal O_p\left( |\mathcal S|\frac{\sqrt{\mathbb E_{\mu}[\rho_t^2(s_t,a_t)]  }}{(1 + \sum_{s} \varepsilon_{t + 1}^{\pi}(s)) \sqrt{n}} \right),
% \end{align}
\begin{align}
& \sum_s |\widetilde \varepsilon_{t + 1}^{\pi}(s)|
\\
\leq
& \frac{ 1 + \widetilde{\mathcal O} \left( |\mathcal S|\sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{|\mathcal S|}{n\eta \eta_t} \right) }{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \sum_{s_t} |\widetilde \varepsilon_{t}^{\pi}(s_t)|\\
& + \frac{1}{1 + \sum_s \varepsilon_{t+ 1}^\pi (s)} \widetilde{\mathcal O}\left( |\mathcal S|\sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \right).
\end{align}
where
\begin{align}
& \sum_s \varepsilon_{t + 1}^{\pi}(s) = \widetilde{\mathcal O}\left( |\mathcal S|\sqrt{\frac{\max_{s}(w_t^2(s))}{n \eta^2}} \right) \\
& + \widetilde{\mathcal O}\left(\sum_s\sum_{s_t}\left( \sqrt{ \frac{\E_\mu[\rho_t^2 | s_t] }{n\eta_t}} + \frac{1}{n\eta \eta_t} \right) \widetilde\varepsilon_{t}^{\pi}(s_t) \right).
\end{align}
\end{theorem}
We provide the detailed proof of Theorem~\eqref{thm:err_prop_2} in Appendix~\ref{app:proof_sec4}. The error propagation of the estimator with self-normalization is quantitatively the same as the estimator without self-normalization. But it strictly reduces the error if $\sum_s \varepsilon_{t + 1}^{\pi} (s) > 0$.

The next Corollary discuss the estimated error $\sum_s |\widehat\varepsilon_{t}^{\pi}(s)|$ based on the Theorems about error propagation. It shows the linear dependence on horizon $H$ if $n$ is large enough.

\begin{corollary}
\label{cor:cor1}
Let $\rho_t(s_t,a_t) \leq 1/\eta$. Let $\widehat \varepsilon_t^{\pi}(s) \coloneqq \widehat d_t^{\pi}(s) - d_t^{\pi}(s)$.

If $n \gg \frac{|S|^2H^2}{\eta^2}$, then with high probability,
\begin{align*}
    \sum_s |\widehat\varepsilon_{t}^{\pi}(s)| = \widetilde{\mathcal O}\left(\frac{H |S|}{\eta \sqrt{n}}\right).
\end{align*}

\note[tx]{We only need $n > \frac{|S|^2H^2}{\eta^2}$, right? We may be able to use $(1 + 1/n)^n < e$ for the error propagation.}

\note[yw]{
\begin{enumerate}
    \item This is what our bounds above imply, suppose that everything also holds in high probability, rather than just $O_p(\cdot)$. We can get the high probability bound trivially if we bound the smallest state probability of the logging policy from below with $\eta_1$.
    \item Even if we can estimate $\E[r_t|s_t,a_t]$ perfectly (and assume boundedness of this quantity), this bound will give a policy evaluation (absolute, rather than MSE) error bound of $O(\frac{H^2|S|}{\eta\sqrt{n}})$.
    \item Let's say the optimal policy is given to us. To what extent can be check it?  The sample complexity to verify that an optimal policy to $\epsilon$ accuracy is using the above $n = O(\frac{H^4S^2}{\eta^2\epsilon^2}).$
    \item If we have concentration, this also imply a trivial off-line learning method that gets $\text{poly}(H,S)$ sample complexity. This is suboptimal, since Chris Dann's result suggests that the optimal sample complexity bound for learning is $
    \frac{H^2SA}{\epsilon^2}$
    It seems like we should be able to improve the bound in terms of the dependence on $H,S$ and $\eta$.
    But we do not really know because we are also constraining ourselves to offline learning.
\end{enumerate}}
\end{corollary}

The detailed proof of Corollary~\ref{cor:cor1} is provided in Appendix~\ref{app:proof_sec4}.

\begin{remark}
Corollary~\ref{cor:cor1} provide an upper bound of estimated error $\sum_s |\widehat\varepsilon_{t}^{\pi}(s)|$ based on its error propagation. Based on that Corollary above, we can obtain an absolute error bound of our estimator for the off-policy policy evaluation problem. If the reward is bounded and we can estimate the reward function $\E[r_t|s_t,a_t]$ perfectly, our bounds on marginalized distribution $d_t^{\mu}(\cdot)$ and $d_t^{\pi}(\cdot)$ will give the off-policy policy evaluation an absolute error bound of $\widetilde{\mathcal O}\left(\frac{H^2|S|}{\eta\sqrt{n}}\right)$.
\end{remark}



% \subsection{Further Theoretical Analysis}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

